Using Containers to Create More Interactive Online Training and Education Materials

Containers are excellent hands-on learning environments for computing topics because they are customizable, portable, and reproducible. The Cornell University Center for Advanced Computing has developed the Cornell Virtual Workshop in high performance computing topics for many years, and we have always sought to make the materials as rich and interactive as possible. Toward the goal of building a more hands-on experimental learning experience directly into web-based online training environments, we developed the Cornell Container Runner Service, which allows online content developers to build container-based interactive edit and run commands directly into their web pages. Using containers along with CCRS has the potential to increase learner engagement and outcomes.

==> readme.tex <==
Note!: this is not really a LaTex file! Do NOT try to compile in overleaf while having this file open.

To generated output for grammarly do e.g.:

pandoc --wrap=none -o doc.txt doc.tex

Also look into https://pandoc.org/filters.html for a possible way to remove references
